Anomaly Detection with Conditioned Denoising Diffusion Models

Traditional reconstruction-based methods have struggled to achieve competitive performance in anomaly detection. In this paper, we introduce Denoising Diffusion Anomaly Detection (DDAD), a novel denoising process for image reconstruction conditioned on a target image. This ensures a coherent restoration that closely resembles the target image. Our anomaly detection framework employs the conditioning mechanism, where the target image is set as the input image to guide the denoising process, leading to a defectless reconstruction while maintaining nominal patterns. Anomalies are then localised via a pixel-wise and feature-wise comparison of the input and reconstructed image. Finally, to enhance the effectiveness of the feature-wise comparison, we introduce a domain adaptation method that utilises nearly identical generated examples from our conditioned denoising process to fine-tune the pretrained feature extractor. The veracity of DDAD is demonstrated on various datasets including MVTec and VisA benchmarks, achieving state-of-the-art results of \(99.8 \%\) and \(98.9 \%\) image-level AUROC respectively.

==> tables/DDAD-n-VisA.tex <==
% \begin{table*}[ht]
% \centering
% \caption{Anomaly Detection Performance (Image AUROC) on VisA \cite{zou2022spot}, based on various denoising steps.} 
% \resizebox{\textwidth}{!}{\begin{tabular}{ccccccccccccccc}
% \toprule
%  \textbf{Categories} &Candle & Capsules &Cashew &Chewing gum &Fryum &Macaroni1 &Macaroni2 &PCB1 &PCB2 &PCB3 &PCB4 &Pipe fryum &Avg\\
%  \midrule
%  \textbf{DDAD-3}  &93.4 & 95.6 &74 &95.4 &86.8 &99.6 &83.7 &81.9 &100 &99.3 &99.4 &95.7 &92.1 \\
%  \textbf{DDAD-5}  &99.9 & 97.8 &90.2 &99.7 &97.6 &99.6 &97.0 &99.6 &99.3 &99.2 &99.3 &99.9 &98.2 \\
%  \textbf{DDAD-10}  &99.9 & 97.9 &98.4 &99.0 &98.8 &100 &99.2 &99.9 &99.2 &100 &99.9 &99.8 &99.3 \\
%  \textbf{DDAD-20}  &99.8 & 99.8 &98.8 &100 &98.2 &100 &99.4 &99.5 &100 &100 &99.3 &99.6 &99.5 \\
% \bottomrule
% \end{tabular}}
% \label{Table:VisA_DDAD-n_Detection_Appendix}
% \end{table*} 



% \begin{table*}[ht]
% \centering
% \caption{Anomaly Localization Performance (Pixel AUROC, PRO) on VisA \cite{zou2022spot}, based on various denoising steps.} 
% \resizebox{\textwidth}{!}{\begin{tabular}{ccccccccccccccc}
% \toprule
%  \textbf{Categories} &Candle & Capsules &Cashew &Chewing gum &Fryum &Macaroni1 &Macaroni2 &PCB1 &PCB2 &PCB3 &PCB4 &Pipe fryum &Avg\\
%  \midrule
%  \textbf{DDAD-3}  &(89.0,66.8)  & (97.8,88.2) &(88.7,81.0) &(91.1,69.0)  &(77.7,76.8) &(94.9,95.5) &(88.8,86.7) &(87.9,76.3) &(97.2,92.4) &(95.8,89.7) &(95.2,83.2) &(77.2, 60.8)  &(90.1 ,80.5) \\
%  \textbf{DDAD-5}  &(98.2,95.6) & (99.3,94.5) &(92.1,83.4) &(92.7,79.4)  &(91.2,91.6) &(99.0,98.6) &(98.4,98.1) &(91.5,89.8)  & (97.5,92.2) &(97.7,94.3)  &(97.3,89.0) & (95.0,81.9)  &(95.8 ,90.7)\\
%  \textbf{DDAD-10} & (98.4,95.2) & (99.6,95.7) &(93.0,80.5) &(97.6,84.4)  &(93.6,93.3) &(99.3,99.1) &(99.2,98.5) &(94.3,94.4) &(97.0,90.6) &(98.1,95.2) &(98.3,92.3) &(96.5,85.2)  &(97.0,92.0)\\
%  \textbf{DDAD-20} &(97.8,95.0) & (99.7,96.4) &(90.4,78.0) & (93.0,79.8)  & (89.5,90.0) &(99.4,99.3) &(99.3,99.5) &(91.9,91.9) &(97.5,91.5) &(98.1,95.4) &(97.4,88.3) &(96.3,85.0)  & (95.8, 90.8) \\
% \bottomrule
% \end{tabular}}
% \label{Table:VisA_DDAD-n_Localization_Appendix}
% \end{table*} 
